Data Dissemination in Cognitive Radio Networks

In this report, we first describe the problem that we are dealing with i.e. data dissemination in multi-hop cognitive radio networks. To address this problem, we propose a channel selection strategy named 'SURF'. We evaluate the proposed channel selection strategy in both single-hop and multi-hop scenarios and compared it with relevant approaches. So far, one technical report and a poster is published as part of this work, while two publications are under review; one is in IEEE Communications Letters and the second one is in IEEE WoWMoM conference. In on-going works sections, we first mention some possible directions in the context of SURF. In addition to that, we mention different research problems that we are planning to deal during the course of this PhD dissertation.

==> chap_tex/abstract.tex <==
%
%   Abstract
%
%\vspace{5mm}


\typeout{*** Abstract ***}
\selectlanguage{english}

\label{chap:abstract}

In this thesis, 

==> chap_tex/bib.tex <==
\typeout{*** Bibliographies ***} \selectlanguage{english}
\def\bibname{References}
\addcontentsline{toc}{chapter}{References}
\lhead[\fancyplain{}{\sl\thepage}]{\fancyplain{}{}}
\chead[\fancyplain{}{\sl References}]{\fancyplain{}{\sl References}}
\rhead[\fancyplain{}{}]{\fancyplain{}{\sl\thepage}}
%\nocite{*}
\bibliographystyle{./style/ieeetr-lui}
%\bibliographystyle{plain}
\bibliography{these}


==> chap_tex/chapter1.tex <==
\typeout{*** Chapter 1 ***}
\label{L:chap1}

\section{Introduction}
Wireless sensor network performance is greatly influenced by the deployment process. The deployment ...

==> chap_tex/conclusion.tex <==
\selectlanguage{english}
\typeout{*** Conclusion ***}

In this chapter we will conclude the thesis and present the future work  

\section{Summary of contributions}
\label{conc:sec1}

In this thesis, we focused on the problems i

==> chap_tex/figures.tex <==
\typeout{*** List of figures ***}

\addcontentsline{toc}{chapter}{List of figures}
\def\listfigurename{List of figures}
\setlength{\parskip}{0mm}

\listoffigures

\lhead[\fancyplain{}{\sl\thepage}]{\fancyplain{}{}}
\chead[\fancyplain{}{\sl List of figures}]{\fancyplain{}{\sl List of
    figures}}
\rhead[\fancyplain{}{}]{\fancyplain{}{\sl\thepage}}


==> chap_tex/introduction.tex <==
\selectlanguage{english}
\typeout{*** Intro ***}

The integration ...

\section{Wireless sensor network architecture}

A wireless sensor network  ...

==> chap_tex/keywords.tex <==
\selectlanguage{english}
\typeout{*** Keywords ***}


\section*{Key Words}

Cognitive Radio Networks.



==> chap_tex/table.tex <==
\typeout{ *** Table of contents ***}

\selectlanguage{english}

%\pagestyle{fancyplain} \headrulewidth        0.1pt \footrulewidth
%0.0pt \plainheadrulewidth   0.0pt \plainfootrulewidth   0.0pt
%\cfoot{} \lhead[\fancyplain{}{\sl\thepage}]{\fancyplain{}{}}
%\chead[\fancyplain{}{\sl Table of contents}]{\fancyplain{}{\sl Table
%of contents}} \rhead[\fancyplain{}{}]{\fancyplain{}{\sl\thepage}}

\ifnumcont\else \setcounter{page}{1}
\pagenumbering{roman} % Numérotation romaine
\fi

\def\contentsname{Table of contents}

\dominitoc
\tableofcontents

\newpage

\thispagestyle{empty} \mbox{}
\newpage


%% ----- Formattage Général

%\pagestyle{fancyplain}
%\renewcommand{\chaptermark}[1]{\markboth{#1}{#1}}
%\renewcommand{\sectionmark}[1]{\markright{\thesection\ \ #1}}
%\lhead[\fancyplain{}{\sl\thepage}]{\fancyplain{}{\sl\rightmark}}
%\chead[\fancyplain{}{\sl\leftmark}]{\fancyplain{}{}}
%\rhead[\fancyplain{}{\sl Chapter
%\thechapter}]{\fancyplain{}{\sl\thepage}}

\ifnumcont\else \setcounter{page}{1} \pagenumbering{arabic} \fi

\def\baselinestretch{1.0}
\normalsize


==> chap_tex/tables.tex <==
\typeout{*** List of tables ***}


\addcontentsline{toc}{chapter}{List of tables}
\def\listtablename{List of tables}
\setlength{\parskip}{0mm}

\listoftables

\lhead[\fancyplain{}{\sl\thepage}]{\fancyplain{}{}}
\chead[\fancyplain{}{\sl List of tables}]{\fancyplain{}{\sl List
    of tables}}
\rhead[\fancyplain{}{}]{\fancyplain{}{\sl\thepage}}





